Logit Standardization in Knowledge Distillation

Knowledge distillation involves transferring soft labels from a teacher to a student using a shared temperature-based softmax function. However, the assumption of a shared temperature between teacher and student implies a mandatory exact match between their logits in terms of logit range and variance. This side-effect limits the performance of student, considering the capacity discrepancy between them and the finding that the innate logit relations of teacher are sufficient for student to learn. To address this issue, we propose setting the temperature as the weighted standard deviation of logit and performing a plug-and-play Z-score pre-process of logit standardization before applying softmax and Kullback-Leibler divergence. Our pre-process enables student to focus on essential logit relations from teacher rather than requiring a magnitude match, and can improve the performance of existing logit-based distillation methods. We also show a typical case where the conventional setting of sharing temperature between teacher and student cannot reliably yield the authentic distillation evaluation; nonetheless, this challenge is successfully alleviated by our Z-score. We extensively evaluate our method for various student and teacher models on CIFAR-100 and ImageNet, showing its significant superiority. The vanilla knowledge distillation powered by our pre-process can achieve favorable performance against state-of-the-art methods, and other distillation variants can obtain considerable gain with the assistance of our pre-process.

==> iccv/section/abstract.tex <==
\begin{abstract}
   %Knowledge distillation transfers the soft labels of a teacher to a student besides the hard target. To achieve that, a \softmax function involving a temperature factor is leveraged to convert logit to probability for both teacher and student. It is widely accepted that the teacher and student share an identical temperature. However, there is no theoretical guarantee for the setting of a shared temperature. Under the assumption of a well-trained student and the condition of a shared temperature, two implicit relations between their logits hold. The first is that a constant shift exists between the teacher's and student's logits. The second is the variances of their logits are the same. This is unexpected as the student of fewer layers is forced to produce the logit of the same magnitude and variance as the cumbersome teacher. To alleviate the side-effect, we show the ratio between their temperatures ideally equals the ratio between the standard deviations of their logits. Therefore, we propose setting the temperature as the weighted standard deviation of logit and forming a \zscore pre-process before \softmax. The pre-process is easily defined and implemented. It can be incorporated into existing logit-based knowledge distillation methods involving temperature and help improve their performance. The proposed pre-process is extensively evaluated for various student and teacher models on CIFAR-100 and ImageNet datasets showing its significant superiority. The vanilla knowledge distillation powered by our pre-process can achieve comparable performance against state-of-the-art methods. A considerable gain is obtained for other methods after the assistance of our pre-process.
   %
   Knowledge distillation involves transferring soft labels from a teacher to a student using a shared temperature-based \softmax function. However, the assumption of a shared temperature between the teacher and student results in the side-effect that the lightweight student is forced to generate logits of the same range and variance as the cumbersome teacher, which can limit the student's performance. 
   %
   To address this issue, we propose setting the temperature as the weighted standard deviation of logit and performing a \zscore pre-process before \softmax. Our key observation is that the ratio between the temperatures of the teacher and student models ideally equals the ratio between the standard deviations of their logits. 
   %
   The pre-process is easily defined and implemented and can improve the performance of existing logit-based knowledge distillation methods involving temperature. We extensively evaluate the proposed method for various student and teacher models on CIFAR-100 and ImageNet, showing its significant superiority. The vanilla knowledge distillation powered by our pre-process can achieve favorable performance against state-of-the-art methods, and other distillation variants can obtain considerable gain with the assistance of our pre-process.
\end{abstract}

==> iccv/section/algorithm.tex <==

\begin{algorithm}[htbp]
% \renewcommand{\thealgocf}{}
    \SetAlgoLined
	\caption{\zscore logit standardization pre-process in knowledge distillation.}\label{alg::zscore}
	\label{alg:algorithm1}
	\KwIn{Transfer set $\D$ with samples of image-label pair $\{\xv_n,\y_n\}_{n=1}^N$, Number of classes $K$, Base Temperature $\tau$, Teacher $f_T$, Student $f_S$, Loss $\Loss$ (e.g., $\KL$ divergence $\Loss_\KL$)}
	\KwOut{Trained student model $f_S$}  
	\BlankLine
	% Assign $\beta_1 = 0.9$, $\beta_2 =0.999$, $\epsilon=1e-8$
	
	% Initialize ;
	
    % $\leftarrow \clip(\x+\z, 0, 1)$
    
	\ForEach{ $(\xv_n,\y_n)$ in $\D$}{
		$\vv_n \leftarrow f_T(\xv_n)$, 
    % 
            $\overline{\vv}_n \leftarrow \frac{1}{K} \sum_{k=1}^K \vv_n^{(k)}$ %\hspace{-0.05\linewidth}%\hspace{0.139\linewidth} 
    
            $\zv_n \leftarrow f_S(\xv_n)$,\hspace{0.0059\linewidth} 
    %
            $\overline{\zv}_n \leftarrow \frac{1}{K} \sum_{k=1}^K \zv_n^{(k)}$

            $\sigma (\vv_n) \leftarrow \left[{\frac{1}{K} \sum_{k=1}^K \left(\vv_n^{(k)} - \overline{\vv}_n\right)^2}\right]^{1/2}$
            
            $\sigma (\zv_n) \leftarrow \left[{\frac{1}{K} \sum_{k=1}^K \left(\zv_n^{(k)} - \overline{\zv}_n\right)^2}\right]^{1/2}$

            $q(\vv_n) \leftarrow \text{\softmaxf} \left[ (\vv_n - \overline{\vv}_n ) / \sigma (\vv_n) / \tau \right]$

            $q(\zv_n) \leftarrow \text{\softmaxf} \left[ (\zv_n - \overline{\zv}_n ) / \sigma (\zv_n) / \tau \right]$

            $q'(\zv_n) \leftarrow \text{\softmaxf} \left( \zv_n\right)$
            
		% Update $f_S$ towards minimizing a weighted sum of $\Loss_{CE}\left(\y_n, q'(\zv_n)\right)$ and $\tau^2 \Loss \left(q(\vv_n), q(\zv_n)\right)$

            Update $f_S$ towards minimizing {\footnotesize $\lambda_{CE}\Loss_{CE}\left(\y_n, q'(\zv_n)\right) + \lambda_{KD}\tau^2 \Loss \left(q(\vv_n), q(\zv_n)\right)$}
            
            % \# Note that the CE loss is abbreviated here for simplicity
	}
\end{algorithm}
% \vspace{-3mm}


==> iccv/section/conclusion.tex <==
\vspace{-1.5mm}
\section{Conclusion}
\vspace{-1.5mm}
In this work, we observe a lack of theoretical support for the global and shared temperature in conventional KD methods. We thus analyze the principle of entropy maximization and come to a conclusion that temperature comes from a flexible Lagrangian multiplier and thus can be defined flexibly. 
%
We then show the ideal ratio between the logit standard deviations of the teacher and student equals to the ratio between defined temperatures. From the observation, we propose a logit \zscore standardization as a pre-process to boost arbitrary logit-based KD methods involving temperature. 
%
Extensive experiments demonstrate the effectiveness of our pre-process method.

==> iccv/section/experiment.tex <==

\vspace{-1.5mm}
\section{Experiments}
\vspace{-1.5mm}
\noindent\textbf{Datasets.} We conduct experiments on CIFAR-100~\cite{krizhevsky2009learning} and ImageNet~\cite{russakovsky2015imagenet}. CIFAR-100~\cite{krizhevsky2009learning} is a common dataset for image classification consisting of 50,000 training and 10,000 validation images. It contains 100 classes and its image size is $32\times 32$. ImageNet~\cite{russakovsky2015imagenet} is a large scale dataset for image classification containing 1,000 categories and around 1.28 million training and 50,000 validation images.

\noindent\textbf{Baselines.} We evaluate the effect of our proposed logit standardization as pre-process for multiple logit-based KD approaches, including KD~\cite{hinton2015distilling}, CTKD~\cite{li2022curriculum}, DKD~\cite{zhao2022decoupled} and MLKD\cite{jin2023multi}. 
We also select various feature-based KD methods inlcuding FitNet~\cite{romero2014fitnets}, RKD~\cite{park2019relational}, CRD~\cite{peng2019correlation}, OFD~\cite{heo2019comprehensive}, ReviewKD~\cite{chen2021distilling}, SimKD~\cite{chen2022knowledge}, and CAT-KD~\cite{guo2023class} for comparison.

\input{iccv/section_tab/tab_imagenet}


% \noindent\textbf{Implementation Details} are attached in the supplementary materials due to page limit.

\noindent\textbf{Implementation Details.} We follow the same experimental settings as previous works~\cite{chen2021distilling,zhao2022decoupled}. For the experiments on CIFAR-100, the optimizer is SGD~\cite{sutskever2013importance} and the epoch number is $240$. The learning rate is set initially 0.01 for MobileNets\cite{howard2017mobilenets,sandler2018mobilenetv2} and ShuffleNets~\cite{zhang2018shufflenet} and 0.05 for other architectures consisting of ResNets~\cite{he2016deep}, WRNs~\cite{zagoruyko2016wide} and VGGs~\cite{simonyan2014very}. 
% The learning rate shrinks by a decay rate of $0.1$ at $150$-th, $180$th and $210$th epochs. For the settings on ImageNet, SGD solver is used and the total epoch number is 100. The learning rate is set to $0.2$ and divided by $10$ at $30$th, $60$th, $90$th epochs. 
All results are reported by taking average over 4 trials. 
More detailed experimental settings are elaborated in the supplementary materials.


\subsection{Main Results}
\vspace{-2mm}


\noindent\textbf{Results on CIFAR-100.} 
We compare the distillation results of different KD methods under various teacher/student settings in Table~\ref{tab:diffStru} and \ref{tab:sameStru}. 
Table~\ref{tab:diffStru} shows the cases where the teacher and student models have distinct structures, while Table~\ref{tab:sameStru} demonstrates the cases where they have the same architecture. 
% Due to page limit, we append more comparisons under other settings of different architectures in the supplementary materials.

We evaluate our pre-process on three logit-based distillation methods. As shown, our \zscore standardization can constantly improve the existing logit-based KD approaches. After applying our pre-process, the vanilla KD~\cite{hinton2015distilling} achieves comparable performance with the state-of–the-art feature-based methods. As the state-of-the-art logit-based method, DKD~\cite{zhao2022decoupled} can also be further boosted by our proposed pre-process. CTKD~\cite{li2022curriculum} is a KD method that can determine sample-wise temperature based on adversarial learning. We combine it with our standardization by leveraging it to predict the base temperature in Alogorithm~\ref{alg::zscore}. As illustrated in tables, student models distilled by CTKD benefits from our pre-process. CTKD can consistently improve KD and on the basis of CTKD, our method further enhances the performance by a significant margin.

\noindent\textbf{Results on ImageNet} of different methods in terms of top-1 and top-5 accuracy are compared in Table.~\ref{tab:imagenet}. Our pre-process can achieve consistent improvement for all the three logit-based methods on the large scale dataset as well. 

\input{iccv/section_tab/tab_ablation-1}

% \subsection{Ablation Studies}
% \vspace{-2mm}

\noindent\textbf{Ablation Studies}
We conduct extensive ablation studies in terms of different configurations of the base temperature and the weight of KD loss $\lambda_{KD}$. The part of results when base temperature is 2 are shown in Table.~\ref{tab:ablation-1}. We can see as the weight of KD loss increases, the vanilla KD where \softmax takes the original logit vectors as input cannot have a considerable performance gain. In contrast, our pre-process of \zscore can achieve a significant enhancement. More ablation studies of other configurations are in the supplementary materials. 

% Our \zscore has a similar idea regarding standard deviation with ATKD~\cite{guo2022reducing}. As shown in Table.~\ref{tab:ablation-1}, our results are consistantly better than $\frac{\zv}{\sigma(\zv)}$. 

The weight of KD loss is set relatively larger than that of CE loss because our pre-process enables better mimicking of students. A large weight of KD makes student focus more on the dark knowledge from teachers instead of hard labels. Another reason of the large KD weight is to compensate the gradient involving \zscore. We give the analysis in the supplementary materials due to page limit.


\input{iccv/section_fig/diff/diff}

\input{iccv/section_fig/tsne/tsne}

\input{iccv/section_tab/tab_various_tea}
% \noindent\textbf{Comparison with ATKD~\cite{guo2022reducing}.} 

\vspace{-1.5mm}
\subsection{Extensions}
\vspace{-1.5mm}

\noindent\textbf{Logit range.} We plot a bar plot in the first row of Fig.~\ref{fig:diff} to show an example of logit range. The second row of Fig.~\ref{fig:diff} illustrates the extent of average logit difference between teacher and student. Without applying our pre-process, the student fails to produce as large logit as the teacher at the target label index (7.5 v.s. 12). The mean average distance between the teacher and student logits also reaches 0.27. The restriction of logit range impedes the student to predict correctly. In contrast, our pre-process breaks the restriction and enables the student to generates the logits of appropriate range for itself. Its effective logit output after standardization on the contrary matches the teacher's nicely. The mean distance of standardized logits also shrinks to 0.18, implying its better mimicking the teacher.



\noindent\textbf{Logit variance.} As illustrated in the first row of Fig.~\ref{fig:diff}, the vanilla KD forces the variance of the student logits approaches the teacher's (3.78 v.s. 3.10). However, our pre-process breaks the shackle and the student logit can have flexible logit variance (0.48 v.s. 3.10), while its standardized logits have the same variance as the teacher (both 0.99).

\noindent\textbf{Feature visualization.} We visualize the the representation of deep features in Fig.~\ref{fig:tsne}. As implied, our pre-process improves the feature separability and discriminability of all the methods including KD~\cite{hinton2015distilling}, CTKD~\cite{li2022curriculum}, and DKD~\cite{zhao2022decoupled}.

% \input{iccv/section_fig/logit/logit}

\input{iccv/section_fig/bivar_hist/b_hist}


\noindent\textbf{Improving distillation for large teacher.} Existing works~\cite{cho2019efficacy,wang2021knowledge,zhao2022decoupled} observe that a bigger teacher model will unnecessarily be a good teacher. The phenomenon implies that the transfer of knowledge from a large teacher is not always as smooth as a small teacher. They provide an explanation on the observation that there exists a capacity gap between cumbersome teachers and lightweight students. 

We interpret the issue as the difficulty of students in mimicking logits of comparable range and variance as teachers. As shown in the bivariate histogram of Fig.~\ref{fig:b_hist-a}, the bigger teacher models like ResNet50 and VGG13 generates the logits of mean closer to zero and smaller standard deviation. The tendency shows that smaller models intrinsically predicts the outputs of larger bias from zero mean and larger variance. Therefore, when students are small, the same tendency remains and they are difficult to produce as compact logits as large teachers in terms of mean and variance. %where the optimization of conventional KD approaches compels students to overcome it with difficulty.

We alleviate the problem by our pre-process. As shown in Table~\ref{tab:various_tea}, our pre-process consistently improves the distillation performance for various teachers of different sizes and capacities. We also show the mimicking goodness of students by a bivariate histogram plot in Fig.~\ref{fig:b_hist-b}. The student distilled by vanilla KD predicts logits apparently deviated from teachers' in terms of logit mean and standard deviation. In contrast, our pre-process enables the student to perfectly matching the teacher in terms of standardized logit mean and standard deviation (see the zoomed-in region at bottom right corner).

% \subsection{Limitation}
% The determination

% \input{iccv/section_tab/tab_imagenet-rn18}
% \input{iccv/section_tab/tab_imagenet-mn2}



==> iccv/section/intro.tex <==
\section{Introduction}
\input{cvpr/cover/fig1.tex}
\input{cvpr/toy_case/toy_case}
The development of deep neural networks (DNN) has revolutionized the field of computer vision in the past decade. However, with increasing performance and capacity, the model size and computational cost of DNN have also been expanding. Despite of a tendency that larger models have greater capacity, many efforts have been made by researchers to cut down model size without sacrificing much accuracy. In addition to designing lightweight models, knowledge distillation (KD) has emerged as a new approach to achieve this goal. It involves transferring the knowledge of a pre-trained heavy model, known as the teacher network, to a small target model, known as the student network. 
%The previous model is commonly called a teacher model and the latter is called student.

Hinton et al.~\cite{hinton2015distilling} firstly proposes distilling a teacher's knowledge to a student by minimizing a Kullback-Leibler (KL) divergence between their predictions. A scaling factor in the \softmax function called temperature $\T$ is introduced to soften the predicted probabilities. From that on, the temperature is set globally beforehand as a hyper-parameter and fixed throughout the entire training, until CTKD~\cite{li2022curriculum} adopts an adversarial learning module to predict sample-wise temperatures for better adapting to sample difficulties. 
However, it still assumes that teacher and student should share common temperatures and disregards the possibility that they have distinct temperatures.
% lacks a theoretical analysis on where the scaling factor of temperature comes from and whether its value can be determined sample-by-sample. 
%

In this work, we derive the general \softmax expression in classification and KD based on the principle of entropy maximization in information theory.
%It implies when estimating unknown probability based on prior constraints, the maximal uncertainty should be maintained to determine a least biased distribution. 
%
In classification, the summation of discrete distribution must equal to one to form a valid probability density, and the expectation of the logits must approach a finite value \cite{jaynes1957information,guo2017calibration}.
%In the case of classification, 
%This finite value is the logit of the target category to ensure the model predicts target class correctly. 
%
In the KD task, we need to consider another constraint that the expectation of student logit should approach that of the teacher's due to the introduction of teacher knowledge. 
%
Therefore, we proposed to apply Lagrangian multipliers to the constrained entropy maximization problem and derive the general expression of \softmax function. The multipliers take the form of temperatures in the \softmax function, and their values are not restricted, allowing for the selection of distinct temperatures on a sample-wise basis for the teacher and student models.

From the derived general \softmax function, we further analyze the drawbacks of shared temperature in traditional KD methods. 
%Given a well-distilled student that mimics the probability prediction of teacher, two relations hold for their logits, reflecting the shackles that compels student to mimic unnecessary properties of teacher. The first relation implies the existence of a constant shift between teacher and student logits. 
%
%% This means the difference between any pair of student logit must match the difference of the corresponding teacher logits.
%
%This regulates the relative value range of student logits matches the range of teacher logits. The other relation indicates that the ratio between the standard deviation of teacher and student logits equals to the ratio between their temperatures. In the setting of shared temperature, the variances of student logits and teacher logits match exactly. 
Considering the capacity gap between lightweight student and cumbersome teacher, the student of fewer layers would produce, with difficulty, the logits of comparable range and variance with teacher.
%
Moreover the knowledge about logit values is unnecessary for student to predict equally accurately as teacher. 
%
%Intuitively, the student can be considered good enough if its predicted logit order matches the result of teacher. 
%As a result, the two relations turn into side-effects for student. 
To address this issue, we propose a \zscore logit standardization as a pre-process before applying \softmax. It maps arbitrary range of logits into a bounded range,
%The standardized value range is of zero mean and finite variance. The inner-relation and rank among logits are also retained due to the monotonicity of the \zscore function. The many-to-one mapping 
and enables student logits to possess arbitrary range and variance and only inner order of teacher logits is learnt.

Our contributions are summarized in three folds
\begin{itemize}
\setlength{\itemsep}{0pt}
\setlength{\parsep}{0pt}
\setlength{\parskip}{0pt}
    \item Based on the principle of entropy maximization in information theory, we leverage Lagrangian multipliers to derive the general expression of \softmax. The temperature parameter in the \softmax comes from the Lagrangian multipliers and can be selected with flexibility on a sample-wise base for student and teacher networks.
    \item We find two intrinsic relations between teacher and student logits in well-distilled models that mimic the predicted probability of the teacher. These relations lead to side-effects that compel the student to learn unnecessary knowledge in terms of logit range and variance from the teacher. To address this problem, we propose a pre-process of logit distillation to facilitate existing logit-based KD approaches. 
    \item We conduct extensive experiments for various teacher and student models on CIFAR-100~\cite{krizhevsky2009learning} and ImageNet~\cite{russakovsky2015imagenet} datasets and demonstrate the superior advantage of the proposed method.
\end{itemize}

==> iccv/section/method.tex <==

% \section{Formulating temperature-scaled \softmax}

% We first dig in the formulation of \softmax in knowledge distillation. 

\section{Background and Notation}
%
Suppose we have a transfer dataset $\D$ containing totally $N$ samples $\{\xv_1,\y_1\},...\{\xv_N,\y_N\}$, where $\xv_n\in \mathbb{R}^{H\times W}$ and $\y_n\in [1,K]$ are the image and label respectively of the $n$-th sample. The notations of $H$, $W$ and $K$ are image height, width and the number of possible classes. Given an input $\{\xv,\y\}$, the teacher model $f_T$ generates a logit vector $\vv\in \mathbb{R}^{1\times K}$. Similarly the student model $f_S$ predicts a logit vector $\zv\in \mathbb{R}^{1\times K}$. Namely, $\zv=f_S(\xv)$ and $\vv=f_T(\xv)$.

It is widely accepted that a \softmax function involving a temperature $\T$ is used to convert the logit vector to probability $q(\zv)$ or $q(\vv)$ such that their $k$-th items have
%
\begin{align}
    q(\zv)^{(k)} &= \frac{\exp(\zv^{(k)}/\T)}{\sum_{m=1}^K \exp(\zv^{(m)}/\T)}\label{eq::sharedProbStu} \\
    q(\vv)^{(k)} &= \frac{\exp(\vv^{(k)}/\T)}{\sum_{m=1}^K \exp(\vv^{(m)}/\T)}\label{eq::sharedProbTea},
\end{align}
%
where $\zv^{(k)}$ and $\vv^{(k)}$ are the $k$-th item of the logit vectors $\zv$ and $\vv$ respectively. A knowledge distillation process is essentially letting $q(\zv)^{(k)}$ mimic $q(\vv)^{(k)}$ for any class and all samples. The objective is realized by minimizing a KL-divergence
%
\begin{equation}\label{eq::KL}
    \Loss_\KL\left(q(\vv)||q(\zv)\right) = \sum_{k=1}^K q(\vv)^{(k)} \log \left(\frac{q(\vv)^{(k)}}{q(\zv)^{(k)}}\right),
\end{equation}
%
which is theoretically equivalent to a cross-entropy loss when optimizing solely on $\zv$,
%
\begin{equation}\label{eq::CE}
    \Loss_\CE\left(q(\vv),q(\zv)\right) = -\sum_{k=1}^K q(\vv)^{(k)} \log {q(\zv)^{(k)}}.
\end{equation}
%
Note that they is empirically nonequivalent as their gradients diverge due to the negative entropy term of $q(\vv)$.

% \vspace{-1.5mm}
\section{Method}

It is widely accepted that $\T$ is shared for teacher and student in Eq.~\ref{eq::sharedProbStu} and Eq.~\ref{eq::sharedProbTea}. However, it lacks a theoretical support or analysis on the setting. It is also not shown whether teacher and student can adopt divergent temperatures. In Sec.~\ref{sec::softmaxCl} and \ref{sec::softmaxKD}, we first give a derivation of the temperature-involved \softmax function in classification and KD based on the entropy-maximization principle in information theory. The result implies the temperatures of student and teacher can be distinct and sample-wisely different. In Sec.~\ref{sec::logit_standard}, we show the explicit relation between their temperatures and present our proposed pre-process of logit standardization.

\subsection{Derivation of \softmax in Classification}\label{sec::softmaxCl}

The \softmax function in classification can be proved to be the unique solution of maximizing entropy subject to the normalization condition of probability and a constraint on the expectation of states in information theory~\cite{jaynes1957information}. The derivation is also leveraged in confidence calibration to formulate temperature scaling~\cite{guo2017calibration}. The derived function involving \softmax is well known as Boltzmann distribution. Suppose we have the following constrained entropy-maximization optimization for a training set $\{\xv_n,\y_n\}_{n=1}^N$ and the teacher model, we have the following objective
%
% \begin{theorem}\label{theorem:1}
% \end{theorem}
%
\begin{equation}\label{eq::objCL}
\begin{split}
    &\max_{q} -\sum_{n=1}^N\sum_{k=1}^K q(\vv_n)^{(k)} \log q(\vv_n)^{(k)} \\
    \textit{s.t. } &\left\{
    \begin{aligned}
        &\sum_{k=1}^K q(\vv_n)^{(k)} = 1, \quad \forall n \\
        & \E_q[\vv_n] = \sum_{k=1}^K \vv_n^{(k)}q(\vv_n)^{(k)} = \vv_n^{(y)}, \quad \forall n.
    \end{aligned} \right.
\end{split}
\end{equation}
%
The first constraint is the requirement of discrete probability density. The second constraint controls the scope of the distribution such that the teacher can accurately predict the target class. If we consider the hard label $\y_n$ as an extremely steep probability distribution $\hat q_n$ whose values are all zero except at the target index $\hat q_n^{(\y_n)}=1$, the second constraint can be rewritten as $\sum_{k=1}^K \vv_n^{(k)}q(\vv_n)^{(k)} = \sum_{k=1}^K \vv_n^{(k)}\hat q_n^{(k)} = \vv_n^{(y_n)}$. This is equivalent to making model mimic the hard probability $\hat q_n$.

By applying Lagrangian multipliers $\alpha_{1,1},...,\alpha_{1,N}$ and $\alpha_{2,1},...,\alpha_{2,N}$, it gives
%
\begin{equation*}
\begin{split}
    \Loss_T &= -\sum_{n=1}^N\sum_{k=1}^K q(\vv_n)^{(k)} \log q(\vv_n)^{(k)} \\
    & + \sum_{n=1}^N \alpha_{1,n} \left(\sum_{k=1}^K q(\vv_n)^{(k)} - 1 \right) \\
    & + \sum_{n=1}^N \alpha_{2,n} \left(\sum_{k=1}^K \vv_n^{(k)}q(\vv_n)^{(k)} - \vv_n^{(\y)}\right).
\end{split}
\end{equation*}
%
Taking the partial derivative with respective to $\alpha_{1,n}$ and $\alpha_{2,n}$ yields back the constraints. In contrast, taking the derivative with respective to $q(\vv_n)^{(k)}$ gives
%
\begin{equation}
    \frac{\partial \Loss_T}{\partial q(\vv_n)^{(k)}} = -1 - \log q(\vv_n)^{(k)} + \alpha_{1,n} + \alpha_{2,n}\vv_n^{(k)},
\end{equation}
%
which leads to the solution by making the derivative equal to zero, 
%
\begin{equation}\label{eq::teacher_prob}
    q(\vv_n)^{(k)} = 
    % e^{\alpha_{2,n}\vv_n^{(k)} + \alpha_{1,n} - 1} = 
    \exp \left(\alpha_{2,n}\vv_n^{(k)}\right) / Z_T,
\end{equation}
%
where $Z_T=\exp \left(1 - \alpha_{1,n} \right) = \sum_{m=1}^K \exp\left(\alpha_{2,n}\vv_n^{(m)}\right)$ is called partition function to fulfill the normalization condition. Note that $\alpha_{2,n}$ has no explicit definite expression and thus its choice can be manually defined. If we set $\alpha_{2,n}=1/\T$, Eq.~\ref{eq::teacher_prob} falls in the conventional expression in KD. When $\alpha_{2,n}=1$ the formulation is the traditional \softmax function commonly used in classification. 

\subsection{Derivation of \softmax in KD}\label{sec::softmaxKD}

Following the idea, we can define a problem of entroty-maximization to formulate the \softmax in KD. For a transfer set $\{\xv_n,\y_n\}_{n=1}^N$ and given a well-trained teacher and its prediction $q(\vv_n)$, we have the objective function for the prediction of student as follows,
%
\begin{equation}\label{eq::objKD}
\begin{split}
    &\max_{q} -\sum_{n=1}^N\sum_{k=1}^K q(\zv_n)^{(k)} \log q(\zv_n)^{(k)} \\
    \textit{s.t. } &\left\{
    \begin{split}
        & \sum_{k=1}^K q(\zv_n)^{(k)} = 1,\quad \forall n \\
        & \sum_{k=1}^K \zv_n^{(k)}q(\zv_n)^{(k)} = \zv_n^{(k)},\quad \forall n \\
        & \sum_{k=1}^K \zv_n^{(k)}q(\zv_n)^{(k)} = \sum_{k=1}^K \zv_n^{(k)}q(\vv_n)^{(k)},\quad \forall n.
    \end{split} \right.
\end{split}
\end{equation}
%
By applying Lagrangian multipliers $\beta_{1,n}$, $\beta_{2,n}$ and $\beta_{3,n}$, 
%
\begin{equation*}
\begin{split}
    \Loss_S &= -\sum_{n=1}^N\sum_{k=1}^K q(\zv_n)^{(k)} \log q(\zv_n)^{(k)} \\
    & + \sum_{n=1}^N \beta_{1,n}\left(\sum_{k=1}^K q(\zv_n)^{(k)} - 1\right) \\
    & + \sum_{n=1}^N \beta_{2,n} \left(\sum_{k=1}^K \zv_n^{(k)}q(\zv_n)^{(k)} - \zv_n^{(\y)} \right) \\
    & + \sum_{n=1}^N \beta_{3,n} \sum_{k=1}^K \zv_n^{(k)} \left(q(\zv_n)^{(k)} - q(\vv_n)^{(k)}\right).
\end{split}
\end{equation*}
%
Taking its derivative with respective to $q(\zv_n)^{(k)}$ gives
%
\begin{equation}
    \frac{\partial \Loss_S}{\partial q(\zv_n)^{(k)}} = -1 - \log q(\zv_n)^{(k)} + \beta_{1,n} + \beta_{2,n}\zv_n^{(k)} + \beta_{3,n} \zv_n^{(k)}.
\end{equation}
%
Suppose $\beta_n=\beta_{2,n}+\beta_{3,n}$ for simplicity and it gives 
%
\begin{equation}\label{eq::student_prob}
    q(\zv_n)^{(k)} = 
    % \exp\left(\beta\zv_n^{(k)} + \beta_{1,n} - 1\right) = 
    \exp \left(\beta_n\zv_n^{(k)}\right) / Z_S,
\end{equation}
%
where $Z_S = \exp(1-\beta_{1,n}) = \sum_{k=1}^K \exp(\beta_n \zv_n^{(k)})$ holds because of the normalization condition of probability density. The formulation in Eq.~\ref{eq::student_prob} has the same structure as Eq.~\ref{eq::teacher_prob}. 

\noindent\textbf{Distinct Temperatures.} Note that the partial derivatives of $\Loss_T $ with respective to $\alpha_{1,n}$ and $\alpha_{2,n}$ lead back to the two constraints respectively in Eq.~\ref{eq::objCL} and they are irrelevant to $\alpha_{1,n}$ and $\alpha_{2,n}$. A similar case holds for Eq.~\ref{eq::objKD}. As a result, no explicit expression of them can be given and thus their values can be manually defined. If we set $\beta_n=\alpha_{2,n}=1/\T$, Eq.~\ref{eq::teacher_prob} and \ref{eq::student_prob} turn to the expressions in KD involving a shared temperature for both student and teacher. In contrast, we can certainly choose $\beta_n\ne \alpha_{2,n}$, implying student and teacher can possess different temperatures.

\noindent\textbf{Sample-wise Temperatures.} It is common to define a global temperature for all samples. Namely for any $n$, $\alpha_{2,n}$ and $\beta_n$ are defined as a constant value. In contrast, they could vary across different samples due to the lack of restrictions on them. It lacks a foundation to choose a global constant value as temperature. As a result, adopting sample-wise various temperatures is allowed.



\subsection{Logit Standardization}\label{sec::logit_standard}

It remains unknown how to choose sample-wise distinct temperatures for teacher and student. We first rewrite the \softmax in Eq.~\ref{eq::student_prob} in a general formulation by introducing two hyper-parameters $a_S$ and $b_S$,
%
\begin{equation*}
    q\left(\zv_n; a_S, b_S\right)^{(k)} = \frac{\exp\left[(\zv_n^{(k)}-a_S)/b_S\right]}{\sum_{m=1}^K \exp\left[(\zv_n^{(m)}-a_S)/b_S\right]},
\end{equation*}
%
where $a_S$ can be cancelled out and does not violate the equality. When $a_S=0,b_s=1/\beta_n$, it yields back the special case in Eq.~\ref{eq::student_prob}. The similar equation for the case of teacher can be written by introducing $a_T$ and $b_T$. In KD task, we aim to choose an appropriate values for the hyper-parameters for both student and teacher.

For a finally well-distilled student, we assume the KL divergence loss reaches minimum and its predicted probability density matches that of teacher, i.e., $\forall k\in [1,K]$, $q(\zv_n; a_S, b_S)^{(k)} = q(\vv_n; a_T, b_T)^{(k)}$. Then for arbitrary pair of indice $i,j\in [1,K]$, it can easily lead to 
%
\begin{align*}
    &\frac{\exp\left[(\zv_n^{(i)}-a_S)/b_S\right]}{\exp\left[(\zv_n^{(j)}-a_S)/b_S\right]} = \frac{\exp\left[(\vv_n^{(i)}-a_T)/b_T\right]}{\exp\left[(\vv_n^{(j)}-a_T)/b_T\right]} \\
    \Rightarrow & \left(\zv_n^{(i)} - \zv_n^{(j)}\right) / b_S = \left(\vv_n^{(i)} - \vv_n^{(j)}\right) / b_T.
\end{align*}
%
By taking a summation across $j$ from $1$ to $K$, we have
%
\begin{equation}\label{eq::logitShift}
    \left( \zv_n^{(i)} - \overline{\zv}_n \right) / b_S = \left( \vv_n^{(i)} - \overline{\vv}_n \right) / b_T,
\end{equation}
%
where $\overline{\zv}_n$ and $\overline{\vv}_n$ are the mean of the student and teacher logit vectors respectively, i.e., $\overline{\zv}_n=\frac{1}{K}\sum_{m=1}^K\zv_n^{(m)}$ (similar and omitted for $\overline{\vv}_n$). By taking the summation of the squared Eq.~\ref{eq::logitShift} across $i$ from $1$ to $K$, we can obtain
%
\begin{equation}\label{eq::logitRatio}
    \frac{\sigma(\zv_n)^2}{\sigma(\vv_n)^2} = \frac{\frac{1}{K}\sum_{i=1}^K\left( \zv_n^{(i)} - \overline{\zv}_n \right)^2 }{\frac{1}{K}\sum_{i=1}^K \left( \vv_n^{(i)} - \overline{\vv}_n \right)^2} = \frac{b_S^2 }{ b_T^2},
\end{equation}
%
where $\sigma$ is the function of standard deviation for an input of vector. 
From Eq.\ref{eq::logitShift} and \ref{eq::logitRatio}, we can describe two properties of a well-distilled student in terms of the logit shift and variance matching. 

\noindent\textbf{Logit shift.} From Eq.\ref{eq::logitShift}, it can be found that a constant shift exists between the logits of student and teacher in arbitrary index under the traditional setting of shared temperature ($b_S=b_T$), i.e.,
%
\begin{equation}\label{eq::shackle1}
    \zv_n^{(i)} = \vv_n^{(i)} + \Delta_n,
\end{equation}
%
where $\Delta_n = \overline{\zv}_n - \overline{\vv}_n$ can be considered as constant for the $n$-th sample. This implies in the traditional KD approach, students are forced to strictly mimic the shifted logit of teachers. Take an extreme case as example where $\vv_n^{(\y)}=10,000$ and $\vv_n^{(1)}=0$. The difference between the corresponding logits of student has to be $\zv_n^{(\y)}-\zv_n^{(1)}=10,000$ as well. Considering the gap of their model size and capacity, students may be unable to produce as wide logit range as teachers. In contrast, 
a student can be considered excellent enough when its logit rank matches teacher, i.e., given the indices that sorts the teacher logits $t_1,...,t_K\in[1,K]$ such that $\vv_n^{(t_1)} \le \cdots \le\vv_n^{(t_K)}$, then $\zv_n^{(t_1)} \le \cdots \le\zv_n^{(t_K)}$ holds. The logit order is the essential knowledge that makes student predict as well as teacher. Such a logit shift is thus a side-effect in conventional KD and a shackle compelling student to generate a difficult but unnecessary result.

\noindent\textbf{Variance matching} From Eq.~\ref{eq::logitRatio}, we come into a conclusion that the ratio between the temperatures of student and teacher equal to the ratio between the standard deviations of their predicted logits for a well-distilled student, i.e.,
%
\begin{equation}\label{eq::shackle2}
    \frac{\sigma(\zv_n)}{\sigma(\vv_n)} = \frac{b_S}{b_T}.
\end{equation}
%
In the setting of temperature sharing in vanilla KD, the student is forced to predict logit such that $\sigma(\zv_n)=\sigma(\vv_n)$. This is another shackle applied to student restricting the standard deviation of its predicted logits. In contrast, since the hyper-parameter comes from Lagrangian multiplier and is flexible to tune, we can define $b_S^* \propto \sigma(\zv_n)$ and $b_T^*\propto \sigma(\vv_n)$. In that way, the equation in Eq.~\ref{eq::shackle2} always holds.

To break the two shackles, we therefore propose setting the hyper-parameters $a_S$, $b_S$, $a_T$ and $b_S$ to be the mean and the weighted standard deviation of their logits respectively, 
%
\begin{equation*}
    q\left(\zv_n; \overline{\zv}_n, \sigma(\zv_n)\right)^{(k)} = \frac{\exp(\tilde \zv_n^{(k)})}{\sum_{m=1}^K \exp(\tilde \zv_n^{(k)})},
\end{equation*}
%
where for succinctness $\tilde \zv_n^{(k)} = (\zv_n^{(k)}-\overline{\zv}_n)/\sigma(\zv_n)/\tau$, forming a weighted \zscore standardization pre-process for student logit. The case for teacher logit is similar and omitted. A base temperature $\tau$ is introduced and shared for both teacher and student models. The \zscore standardization has at least four advantages, i.e., zero mean, finite standard deviation, monotonicity and boundedness.

\noindent\textbf{Zero mean.} The mean of standardized vector can be shown to be zero (the proof is left in the supplementary materials). In previous works~\cite{hinton2015distilling,guo2022reducing}, a zero mean is assumed and usually empirically violated. In contrast, the \zscore function intrinsically enables a zero mean.

\input{iccv/section/algorithm.tex}


\noindent\textbf{Finite standard deviation.} The standard deviation of the weighted \zscore output can be shown equal to $1/\tau$ (the proof is in the supplementary materials). The property makes the standardized student and teacher logit map to an identical Gaussian-like distribution with zero mean and standard deviation of definite value. The mapping is many-to-one, meaning that its reverse is indefinite. The variance and value range of original student logit vector $\zv_n$ is thereby free of restriction. 



\noindent\textbf{Monotonicity.} It is easy to show that \zscore is a linear transformation function and thus lies in monotonic functions. This property ensures that the transformed student logit remains the same rank as the original one, i.e., given the indices that sorts the original logits $t_1,...,t_K\in[1,K]$ such that $\zv_n^{(t_1)} \le \cdots \le\zv_n^{(t_K)}$, then $\tilde \zv_n^{(t_1)} \le \cdots \le \tilde \zv_n^{(t_K)}$ holds. The dark knowledge of teacher in the format of logit order can thus be retained and transferred to student.


\input{iccv/section_tab/tab_diffStru-1}
\input{iccv/section_tab/tab_sameStru}


\noindent\textbf{Boundedness.} The standardized logit can be shown bounded within $[-\sqrt{K-1}/\tau, \sqrt{K-1}/\tau]$. Let $\overline{\zv}^*_n = \frac{1}{K-1}\sum_{m\ne t_0}^K \zv_n^{(m)}$ for an arbitrary index $t_0$, then we have
%
{\begin{small}
\begin{align*}
    &\sum_{k=1}^K \left( \zv_n^{(k)} - \overline{\zv}_n\right)^2 = \sum_{k\ne t_0}^K \left(\zv_n^{(k)} - \overline{\zv}^*_n\right)^2 
     + \frac{K}{K-1} \left( \zv_n^{(t_0)} - \overline{ \zv}_n\right)^2 \\
     & \Rightarrow \sigma(\zv_n)^2 \ge  \frac{1}{K-1} \left( \zv_n^{(t_0)} - \overline{ \zv}_n\right)^2\\
     & \Rightarrow \left|\tilde \zv_n^{(t_0)}\right| = \left|(\zv_n^{(t_0)}-\overline{\zv}_n) / \sigma(\zv_n) / \tau\right| \le \left|\sqrt{K-1} / \tau\right|.
\end{align*}
\end{small}}
%
This property ensures the value range of standardized logit to be bounded. Compared to traditional KD, it is achievable to control the range of logit and avoid extremely large exponential value. To this end, we define a base temperature to control the range. 

The pseudo-code of the proposed logit standardization pre-process is illustrated in Algorithm~\ref{alg::zscore}.

% Thanks to the property, the constraint in Eq.~\ref{eq::shackle2} is intrinsically fulfilled because .


% It is well known \softmax is a normalization transformation function to convert logits to probability. We expect the magnitude gap of the logit vectors $\zv_n$ and $\vv_n$ does not affect the optimization in knowledge distillation. 

% Suppose when a perfect student model is trained to exactly mimic a teacher, it generates exactly the same probability identical to teacher's predictions for a given input $\xv_n$, i.e., $q(\zv_n)^{(k)} = q(\vv_n)^{(k)}, \forall k\in [1,K]$. For two arbitrary indices $i,j\in [1,K]$, we can write the ratio between the items within the prediction
% %
% \begin{equation}
%     \frac{q(\zv_n)^{(i)}}{q(\zv_n)^{(j)}} = e^{\beta_n \left(\zv_n^{(i)} - \zv_n^{(i)}\right)},\ \frac{q(\vv_n)^{(i)}}{q(\vv_n)^{(j)}} = e^{\alpha \left(\vv_n^{(i)} - \vv_n^{(i)}\right)}
% \end{equation}
% %
% By $q(\zv_n)^{(k)} = q(\vv_n)^{(k)}$, we have 
% %
% \begin{equation}
%     {\beta_n \left(\zv_n^{(i)} - \zv_n^{(j)}\right)} = {\alpha \left(\vv_n^{(i)} - \vv_n^{(j)}\right)}.
% \end{equation}
% %
% When $\alpha=\beta_n=1/\T$ is set in KD, Ii can easily yield, 
% %
% \begin{equation}
%     \zv_n^{(i)} = \vv_n^{(i)} + \Delta_i,
% \end{equation}
% %
% where $\Delta_i = \E[{\zv_n}] - \E[{\vv_n}]$, $\E[{\zv_n}] = \sum_{n=1}^{K} \zv_n^{(j)} / K$ and $\E[{\vv_n}] = \sum_{n=1}^{K} \vv_n^{(j)} / K$. 

% The relation in Eq.~\ref{eq:logitShift} is an implicit result when we define an shared temperature for the teacher and student. When an assumption that $\E[{\zv_n}]=0$ and $\E[{\vv_n}]=0$ holds, it degenerate to forcing $\zv_n^{(i)}$ approach $\vv_n^{(i)}$, which is inline with the claim in \cite{hinton2015distilling}.

% From Eq.~\ref{eq:logitShift}, we can find that the student logits of an ideal student model will be shifted from the teacher logits by a margin of constant value. Considering a gap between model capacities and complexities between teacher and student, a student of fewer layers may face difficulty in producing logits of the same magnitude as the teacher. A validation experiment is conducted to show the existence of such a gap in Sec.~\ref{}.

% To alleviate the magnitude gap of logits, $\beta_n$ and $\alpha$ can be .

\noindent\textbf{A Toy Case} 
is shown in Fig.~\ref{fig:toy_case} where the conventional logit-based KD setting of shared that temperature may lead to a wrong evaluation of student performance.

==> iccv/section/relatedWorks.tex <==
\section{Related Work}

Knowledge distillation~\cite{hinton2015distilling} is designed to transfer the ``dark'' knowledge from a cumbersome teacher model to a lightweight student model. By learning from the soft labels of teacher, student can achieve better performance than training on hard target only. The traditional method trains a student by minimizing a difference (KL divergence) between its predicted probability and the teacher's. The prediction of probability is commonly approximated by the \softmax of logit output. KD algotithms can be classficied into three types, logit-based~\cite{chen2020online,hinton2015distilling,huang2022knowledge,li2020online,mirzadeh2020improved,zhang2018deep,zhao2022decoupled,jin2023multi}, feature-based~\cite{chen2022knowledge,chen2021distilling,heo2019comprehensive,lin2022knowledge,romero2014fitnets,tian2019contrastive,yim2017gift,ahn2019variational,li2021online,liu2019structured,guo2023class} and relation-based~\cite{park2019relational,peng2019correlation,li2022knowledge,tung2019similarity,yang2021knowledge} methods. 

A temperature is introduced to flatten the probabilities in logit-based methods. Several works~\cite{chandrasegaran2022revisiting,hinton2015distilling,liu2022meta} explore its properties and effects. They reach an identical conclusion that temperature controls how much attention student pays on those logits more negative than average. A very low temperature makes student ignore other logits and instead mainly focus on the largest logit of teacher. However, they do not discuss why teacher and student share a globally predefined temperature. It was unknown whether temperature can be determined in an instance-wise level. CTKD~\cite{li2022curriculum} firstly propose predicting sample-wise temperature by leveraging adversarial learning. 
However, it assumes that teacher and student should share temperatures.
% a theoretical analysis on why sample-wise temperature is valid is not presented. 
It was still undiscovered whether teacher and student can have divergent temperatures. 
%
ATKD~\cite{guo2022reducing} designs a sharpness metric and chooses adaptive temperature by reducing the sharpness gap between teacher and student. However, they omit the theoretical support for distinct temperatures for teachers and students. Besides their assumption of zero logit mean relies on numerical approximation and limits its performance.
%
In this work, we give an analytical derivation based on entropy-maximization principle, showing that student and teacher do not necessarily share a temperature. We also show for a well trained student the ratio between its ideal temperature and the teacher's is proportional to the standard deviations of their logits. Based on the findings, the introduction of temperature can transformed into a weighted \zscore standardization of logit.

% \subsection{Knowledge Distillation}


% \subsection{Probability Calibration}

% \subsection{Information Theory Related to Knowledge Distillation}


==> iccv/section_fig/bivar_hist_ctkd_dkd/bivar_hist_ctkd_dkd.tex <==

\begin{figure}[t]
% \footnotesize
\begin{center}
% \captionsetup[subfloat]{labelsep=none,format=plain,labelformat=empty}
   \subfloat[Teacher and student distilled by CTKD only and CTKD with ours]{\label{fig:b_hist2-a}\includegraphics[trim=0 60mm 0 0,clip,width=1.\linewidth]{iccv/section_fig/bivar_hist_ctkd_dkd/h_dist_ctkd.pdf}}

% \vspace{-3mm}

   \subfloat[Teacher and student distilled by DKD only and DKD with ours]{\label{fig:b_hist2-b}\includegraphics[trim=0 60mm 0 0,clip,width=1.\linewidth]{iccv/section_fig/bivar_hist_ctkd_dkd/h_dist_dkd.pdf}}
   
   \subfloat[Teacher and student distilled by MLKD only and MLKD with ours]{\label{fig:b_hist2-c}\includegraphics[trim=0 60mm 0 0,clip,width=1.\linewidth]{iccv/section_fig/bivar_hist_ctkd_dkd/h_dist_mlkd.pdf}}
\end{center}
\vspace{-3mm}
   \caption{The bivariate histogram of logit mean and logit standard deviation for multiple models on CIFAR-100. }
\label{fig:b_hist2}
% \vspace{-5.5mm}
\end{figure}

==> iccv/section_fig/cover/fig1.tex <==

\begin{figure}[t]
\begin{center}
   \subfloat[Vanilla KD]{\includegraphics[width=0.49\linewidth]{section_fig/cover/1_.eps}}
   \hfill
   \subfloat[KD with logit standardization]{\includegraphics[width=0.49\linewidth]{section_fig/cover/2_.eps}}
\end{center}
   \vspace{-5mm}
   \caption{Vanilla knowledge distillation implicitly forces a constant distance between the logits of teacher and student. It is an unnecessary side-effect because only the order of logits matters in classification and is essential to transfer in distillation. Considering the capacity gap between them, it would also be difficult for a lightweight student to produce logits of the same magnitude as a cumbersome teacher. In contrast, the proposed pre-process of \zscore logit standardization alleviates the side-effect. The standardized logits of student intrinsically share a comparable magnitude with teacher's, while its original logits can have arbitrary magnitude. Due to the monotonicity of standardization, student can efficiently learn the logit order from teacher, without being forced to strictly mimic its logit.}
   \vspace{-4mm}
\label{fig:cover}
\end{figure}

==> iccv/section_fig/diff_ctkd_dkd/diff.tex <==

\begin{figure}[t]
% \footnotesize
\begin{center}
% \captionsetup[subfloat]{labelsep=none,format=plain,labelformat=empty}
   \subfloat[Vanilla CTKD\\ Mean: 0.37, Max: 3.19.]{\label{fig::diff2_kd}\includegraphics[width=0.333\linewidth]{iccv/section_fig/diff_ctkd_dkd/ctkd/heatkd.png}}
   \hfill
   \subfloat[Ours w/o \zscore\\ Mean: 0.94, Max: 7.39.]{\label{fig::diff2_wo_stand}\includegraphics[width=0.333\linewidth]{iccv/section_fig/diff_ctkd_dkd/ctkd/heatkdours1.png}}
   \hfill
   \subfloat[Ours w/ \zscore\\ Mean: 0.09, Max:0.60.]{\label{fig::diff2_w_stand}\includegraphics[width=0.333\linewidth]{iccv/section_fig/diff_ctkd_dkd/ctkd/heatkdours2.png}}
   
% \vspace{-4mm}
   \subfloat[Vanilla DKD\\ Mean: 0.13, Max: 0.99.]{\label{fig::diff3_kd}\includegraphics[width=0.333\linewidth]{iccv/section_fig/diff_ctkd_dkd/dkd/heatkd.png}}
   \hfill
   \subfloat[Ours w/o \zscore\\ Mean: 0.54, Max: 4.35.]{\label{fig::diff3_wo_stand}\includegraphics[width=0.333\linewidth]{iccv/section_fig/diff_ctkd_dkd/dkd/heatkdours1.png}}
   \hfill
   \subfloat[Ours w/ \zscore\\ Mean: 0.08, Max:0.38.]{\label{fig::diff3_w_stand}\includegraphics[width=0.333\linewidth]{iccv/section_fig/diff_ctkd_dkd/dkd/heatkdours2.png}}
   
% \vspace{-4mm}
   \subfloat[Vanilla MLKD\\ Mean: 0.23, Max: 2.75.]{\label{fig::diff4_kd}\includegraphics[width=0.333\linewidth]{iccv/section_fig/diff_ctkd_dkd/mlkd/heatmlkd.png}}
   \hfill
   \subfloat[Ours w/o \zscore\\ Mean: 0.18, Max: 1.91.]{\label{fig::diff4_wo_stand}\includegraphics[width=0.333\linewidth]{iccv/section_fig/diff_ctkd_dkd/mlkd/heatmlkdours1.png}}
   \hfill
   \subfloat[Ours w/ \zscore\\ Mean: 0.06, Max:0.44.]{\label{fig::diff4_w_stand}\includegraphics[width=0.333\linewidth]{iccv/section_fig/diff_ctkd_dkd/mlkd/heatmlkdours2.png}}
\end{center}
\vspace{-3.mm}
   \caption{The heatmaps of the average logit difference between the teacher and student. The \textbf{1st Row} is for CTKD, \textbf{2nd Row} is for DKD and \textbf{3rd Row} is for MLKD. 
   Our pre-process indeed enables the student to generate the logits of divergent range from the teacher as shown in \ref{fig::diff2_wo_stand}, \ref{fig::diff3_wo_stand}\&\ref{fig::diff4_wo_stand}, while its standardized logits (\ref{fig::diff2_w_stand}, \ref{fig::diff3_w_stand}\&\ref{fig::diff4_w_stand}) are more closer to the teacher's than vanilla CTKD (\ref{fig::diff2_kd}), DKD (\ref{fig::diff3_kd}) and MLKD (\ref{fig::diff4_kd}).}
\label{fig:diff23}
% \vspace{-4mm}
\end{figure}

==> iccv/section_fig/logit/logit.tex <==

\begin{figure}[t]
% \footnotesize
\begin{center}
   \subfloat[Vanilla KD]{\label{fig::diff_kd}\includegraphics[width=0.333\linewidth]{iccv/section_fig/logit/kd.png}}
   \hfill
   \subfloat[Ours w/o \zscore]{\label{fig::diff_wo_stand}\includegraphics[width=0.333\linewidth]{iccv/section_fig/logit/kdours2.png}}
   \hfill
   \subfloat[Ours w/ \zscore]{\label{fig::diff_w_stand}\includegraphics[width=0.333\linewidth]{iccv/section_fig/logit/kdours.png}}
\end{center}
   \caption{The heatmap of the average logit difference between teacher ResNet32$\times$4 and student ResNet8$\times$4. Our pre-process indeed enables the student to generate the logits of divergent range from the teacher as shown in \ref{fig::diff_wo_stand}, while its effective logits (\ref{fig::diff_w_stand}) are more closer to the teacher's than vanilla KD (\ref{fig::diff_kd}).}
\label{fig:diff}
\end{figure}

==> iccv/section_fig/rebuttal/rebuttal_traj_1.tex <==

\begin{figure}[t]
% \footnotesize
\setlength{\fboxrule}{0.3pt}
\setlength{\fboxsep}{0.mm} 
\begin{center}
\fbox{
\hspace{-5mm}
\stackinset{l}{25pt}{t}{29pt}{
\fbox{\includegraphics[trim=10 545 1015 120,clip,scale=1,width=0.22\linewidth]{iccv/section_fig/rebuttal/pit.pdf}}
}
{
  \stackinset{r}{20pt}{b}{6pt}{
        \fbox{\includegraphics[trim=261 265 35 255,clip,width=0.6\linewidth]{iccv/section_fig/rebuttal/pit_zoom2.pdf}}
          }{
  \begin{annotationimage}{trim=261 265 35 255,clip,scale=1.,width=1\linewidth}{iccv/section_fig/rebuttal/pit.pdf}
    \node[fill opacity=1, fill=red!10] at (0.09,0.9) {\tiny PiT-Ti};
    \draw[black] (0.75,0.79) rectangle (0.99,0.95);
    \draw [black] (0.32, 0.617) -- (0.75, 0.79);
    \draw [black] (0.911, 0.617) -- (0.99, 0.79);
    \end{annotationimage}
    }}
    \hspace{-3.mm}
}

\fbox{
\hspace{-5mm}
\stackinset{l}{25pt}{t}{29pt}{
\fbox{\includegraphics[trim=10 545 1015 120,clip,scale=1,width=0.22\linewidth]{iccv/section_fig/rebuttal/pvt.pdf}}
}
{
  \stackinset{r}{20pt}{b}{6pt}{
        \fbox{\includegraphics[trim=261 265 35 255,clip,width=0.6\linewidth]{iccv/section_fig/rebuttal/pvt_zoom2.pdf}}
          }{
  \begin{annotationimage}{trim=261 265 35 255,clip,scale=1.,width=1\linewidth}{iccv/section_fig/rebuttal/pvt.pdf}
    \node[fill opacity=1, fill=red!10] at (0.09,0.9) {\tiny PVT-Ti};
    \draw[black] (0.75,0.79) rectangle (0.99,0.95);
    \draw [black] (0.32, 0.617) -- (0.75, 0.79);
    \draw [black] (0.911, 0.617) -- (0.99, 0.79);
    \end{annotationimage}
    }}
    \hspace{-3.mm}
}
    % \end{minipage}
\end{center}
\vspace{-6.5mm}
   \caption{\footnotesize Top-1 validation accuracy on CIFAR-100 for PiT-Ti\&PVT-Ti.}%$\sum\vv-\zv$ for KD and $\sum\tilde\vv-\tilde\zv$ for Ours.}
\label{fig:rebuttal_trajectory}
\vspace{-6mm}
\end{figure}

==> iccv/section_fig/rebuttal/rebuttal_traj_2.tex <==

\begin{figure}[t]
% \footnotesize
\setlength{\fboxrule}{0.3pt}
\setlength{\fboxsep}{0.mm} 
\begin{center}
    \hspace{-2.5mm}
    \begin{minipage}{0.28\linewidth}
        \centering
    \subfloat{\label{fig::acc_trajectory}\includegraphics[width=1\linewidth]{iccv/section_fig/rebuttal/accuracy_trajectory.pdf}}
   \hfill
    \subfloat{\label{fig::loss_trajectory}\includegraphics[width=1\linewidth]{iccv/section_fig/rebuttal/loss_trajectory.pdf}}
    % \subcaption{RN32\(\times\)4-}
    \end{minipage}
    % \begin{minipage}[b]{1\linewidth}
        % \centering
\hspace{-2mm}
\begin{minipage}{0.72\linewidth}
\fbox{
\hspace{-5mm}
\stackinset{l}{22pt}{b}{6pt}{
\fbox{\includegraphics[trim=10 555 1015 120,clip,scale=1,width=0.28\linewidth]{iccv/section_fig/rebuttal/pit.pdf}}
}
{
  \stackinset{r}{2pt}{b}{6pt}{
        \fbox{\includegraphics[trim=261 265 35 255,clip,width=0.6\linewidth]{iccv/section_fig/rebuttal/pit_zoom2.pdf}}
          }{
  \begin{annotationimage}{trim=261 265 35 255,clip,scale=1.,width=1\linewidth}{iccv/section_fig/rebuttal/pit.pdf}
    \node[fill opacity=1, fill=red!10] at (0.09,0.9) {\tiny PiT-Ti};
    \draw[black] (0.405,0.79) rectangle (1,0.99);
    \draw [black] (0.388, 0.725) -- (0.405, 0.79);
    \draw [black] (0.989, 0.725) -- (1, 0.79);
    \end{annotationimage}
    }}
    \hspace{-2.5mm}
}

\fbox{
\hspace{-5mm}
\stackinset{l}{22pt}{b}{6pt}{
\fbox{\includegraphics[trim=10 555 1015 120,clip,scale=1,width=0.28\linewidth]{iccv/section_fig/rebuttal/pvt.pdf}}
}
{
  \stackinset{r}{2pt}{b}{6pt}{
        \fbox{\includegraphics[trim=261 265 35 255,clip,width=0.6\linewidth]{iccv/section_fig/rebuttal/pvt_zoom2.pdf}}
          }{
  \begin{annotationimage}{trim=261 265 35 255,clip,scale=1.,width=1\linewidth}{iccv/section_fig/rebuttal/pvt.pdf}
    \node[fill opacity=1, fill=red!10] at (0.09,0.9) {\tiny PVT-Ti};
    \draw[black] (0.405,0.79) rectangle (1,0.99);
    \draw [black] (0.388, 0.725) -- (0.405, 0.79);
    \draw [black] (0.989, 0.725) -- (1, 0.79);
    \end{annotationimage}
    }}
    \hspace{-2.5mm}
}
% \subcaption{Test Top-1 Acc.}
\end{minipage}
 \hspace{-1mm}
\end{center}
\vspace{-6.mm}
   \caption{\textbf{Left}: Accuracy \& loss of RN32\(\times\)4-RN8\(\times\)4. \textbf{Right}: Top-1 validation accuracy on CIFAR-100 for PiT-Ti \& PVT-Ti.}%$\sum\vv-\zv$ for KD and $\sum\tilde\vv-\tilde\zv$ for Ours.}
\label{fig:rebuttal_trajectory}
\vspace{-2.mm}
\end{figure}

% \fbox{
% \hspace{-5mm}
% \stackinset{l}{25pt}{t}{29pt}{
% \fbox{\includegraphics[trim=10 545 1015 120,clip,scale=1,width=0.22\linewidth]{iccv/section_fig/rebuttal/pvt.pdf}}
% }
% {
%   \stackinset{r}{20pt}{b}{6pt}{
%         \fbox{\includegraphics[trim=261 265 35 255,clip,width=0.6\linewidth]{iccv/section_fig/rebuttal/pvt_zoom2.pdf}}
%           }{
%   \begin{annotationimage}{trim=261 265 35 255,clip,scale=1.,width=1\linewidth}{iccv/section_fig/rebuttal/pvt.pdf}
%     \node[fill opacity=1, fill=red!10] at (0.09,0.9) {\tiny PVT-Ti};
%     \draw[black] (0.75,0.79) rectangle (0.99,0.95);
%     \draw [black] (0.32, 0.617) -- (0.75, 0.79);
%     \draw [black] (0.911, 0.617) -- (0.99, 0.79);
%     \end{annotationimage}
%     }}
%     \hspace{-3.mm}
% }

==> iccv/section_fig/rebuttal/rebuttal_trajectory.tex <==

\begin{figure}[t]
% \footnotesize
\begin{center}
    \subfloat{\label{fig::acc_trajectory}\includegraphics[width=0.333\linewidth]{iccv/section_fig/rebuttal/accuracy_trajectory.png}}
   \hfill
    \subfloat{\label{fig::loss_trajectory}\includegraphics[width=0.333\linewidth]{iccv/section_fig/rebuttal/loss_trajectory.png}}
   \hfill
    \subfloat{\label{fig::logit_diff_trajectory}\includegraphics[width=0.333\linewidth]{iccv/section_fig/rebuttal/logit_diff_trajectory.png}}
\end{center}
\vspace{-7.5mm}
   \caption{Accuracy, loss and logit distance during training. Logit distance is computed by averaging the summation of logit distance. Note that $\lambda_{KD}$ is 9 for ours and 0.9 for KD.}%$\sum\vv-\zv$ for KD and $\sum\tilde\vv-\tilde\zv$ for Ours.}
\label{fig:rebuttal_trajectory}
\vspace{-6mm}
\end{figure}

==> iccv/section_tab/tab_ablation-2.tex <==
% Table generated by Excel2LaTeX from sheet 'ablation'
\begin{table}[t]
\footnotesize
\tabcolsep=0.0mm
  \centering
  \caption{The ablation studies under different settings in \zscore. The base temperature $\tau$ is set to be 1. By default $\lambda_{CE}=0.1$. The logit vector of teacher $\vv_n$ and student $\zv_n$ are abbreviated as $\zv$ for succinctness. The teacher and student are ResNet32$\times$4 and ResNet8$\times$4.}
  \vspace{-3mm}
    \begin{tabular}{c|cccc}
    \toprule
    \makebox[0.07\textwidth][c]{$\lambda_{KD}$} & \makebox[0.09\textwidth][c]{$\zv$ (KD)}     & \makebox[0.09\textwidth][c]{$\zv-\overline \zv$} & \makebox[0.09\textwidth][c]{$\frac{\zv}{\sigma(\zv)}$} & \makebox[0.09\textwidth][c]{$\frac{(\zv-\overline \zv)}{\sigma(\zv)}$ (Ours)} \\
    \midrule
    0.9     & 73.09 & 72.60 & 74.81 & 74.96 \\
    3.0     & 73.79 & 73.65 & 75.89 & 75.85 \\
    6.0     & 73.91 & 73.87 & 75.97 & 76.31 \\
    9.0     & 73.67 & 73.97 & 75.61 & 76.23 \\
    12.0    & 73.60 & 74.00 & 75.89 & 76.11 \\
    15.0    & 73.19 & 73.20 & 75.72 & 75.91 \\
    18.0    & 72.48 & 72.95 & 75.65 & 75.72 \\
    \bottomrule
    \end{tabular}%
  \label{tab:ablation-2}%
  % \vspace{-2mm}
\end{table}%


==> iccv/section_tab/tab_ablation-3.tex <==
% Table generated by Excel2LaTeX from sheet 'ablation'
\begin{table}[t]
\footnotesize
\tabcolsep=0.0mm
  \centering
  \caption{The ablation studies under different settings in \zscore. The base temperature $\tau$ is set to be 4. By default $\lambda_{CE}=0.1$. The logit vector of teacher $\vv_n$ and student $\zv_n$ are abbreviated as $\zv$ for succinctness. The teacher and student are ResNet32$\times$4 and ResNet8$\times$4.}
  \vspace{-3mm}
    \begin{tabular}{c|cccc}
    \toprule
    \makebox[0.07\textwidth][c]{$\lambda_{KD}$} & \makebox[0.09\textwidth][c]{$\zv$ (KD)}     & \makebox[0.09\textwidth][c]{$\zv-\overline \zv$} & \makebox[0.09\textwidth][c]{$\frac{\zv}{\sigma(\zv)}$} & \makebox[0.09\textwidth][c]{$\frac{(\zv-\overline \zv)}{\sigma(\zv)}$ (Ours)} \\
    \midrule
    0.9     & 73.76 & 73.61 & 73.03 & 73.83 \\
    3.0     & 74.07 & 74.09 & 74.15 & 74.33 \\
    6.0     & 74.14 & 73.93 & 76.11 & 76.40 \\
    9.0     & 74.19 & 74.24 & 76.17 & 76.54 \\
    12.0    & 73.96 & 73.97 & 76.12 & 76.39 \\
    15.0    & 73.08 & 73.85 & 76.14 & 76.38 \\
    18.0    & 69.98 & 70.84 & 76.18 & 76.43 \\
    \bottomrule
    \end{tabular}%
  \label{tab:ablation-3}%
  % \vspace{-4mm}
\end{table}%


==> iccv/section_tab/tab_diffStru-2.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table}[t]
\footnotesize
\tabcolsep=0.65mm
  \centering
  \caption{The Top-1 Accuracy (\%) of different knowledge distillation methods on the validation set of CIFAR-100~\cite{krizhevsky2009learning}. The teacher and student have distinct architectures. The KD methods are sorted by the types, i.e., feature-based and logit-based. We apply our logit standardization to the existing logit-based methods and use $\Delta$ to show its performance gain. The values in {\color{blue}blue} denote slight enhancement and those in {\color{red}red} non-trivial enhancement no less than $0.15$. The best and second best results are in \textbf{bold} and \underline{underlined} respectively.}
  \vspace{-3mm}
    \begin{tabular}{llccc}
    \toprule
    \multirow{4}{*}{Type} & \multirow{2}{*}{Teacher} & \makebox[0.09\textwidth][c]{ResNet32$\times$4} & \makebox[0.09\textwidth][c]{ResNet32$\times$4} & \makebox[0.09\textwidth][c]{WRN-40-2} \\
          &       & 79.42 & 79.42 & 75.61 \\
          & \multirow{2}{*}{Student} & SHN-V1 & VGG8  & SHN-V1 \\
          &       & 70.50 & 70.36 & 70.50 \\
    \midrule
    \multirow{8}{*}{Feature} & FitNet~\cite{romero2014fitnets} & 73.59 & 72.91 & 73.73 \\
          & AT~\cite{zagoruyko2017paying} & 71.73 & 72.74 & 73.32 \\
          & RKD~\cite{park2019relational}   & 72.28 & 72.84 & 74.21 \\
          & CRD~\cite{tian2019contrastive}   & 75.11 & 73.54 & 76.05 \\
          & OFD~\cite{heo2019comprehensive}   & 75.98 & 73.85 & 75.85 \\
          & ReviewKD~\cite{chen2021distilling} & 77.45 & 74.35 & 77.14 \\
          & SimKD~\cite{chen2022knowledge} & 77.18 & 75.76 & 75.65 \\
          & CAT-KD~\cite{guo2023class} & \textbf{78.26} & \underline{75.92} & 77.35 \\
    \midrule
    \multirow{13}{*}{Logit} & KD~\cite{hinton2015distilling}    & 74.07 & 72.73 & 74.83 \\
          & KD+Ours & 74.44 & 73.23 & 75.64 \\
          & $\Delta$ & {\color{red}0.37}  & {\color{red}0.50}  & {\color{red}0.81} \\
\cmidrule{2-5}          & KD+CTKD~\cite{li2022curriculum}  & 74.71 & 72.47 & 75.64 \\
          & KD+CTKD+Ours & 74.85 & 73.51 & 76.32 \\
          & $\Delta$ & {\color{blue}0.14}  & {\color{red}1.04}  & {\color{red}0.68} \\
\cmidrule{2-5}          & DKD~\cite{zhao2022decoupled}   & 76.45 & 74.48 & 76.70 \\
          & DKD+Ours & 76.77 & 74.61 & 76.95 \\
          & $\Delta$ & {\color{red}0.32}  & {\color{blue}0.13}  & {\color{red}0.25} \\
\cmidrule{2-5}          & MLKD~\cite{jin2023multi}   & 77.18 & 74.58 & \underline{77.44} \\
          & MLKD+Ours & \underline{78.15} & \textbf{75.98} & \textbf{78.28} \\
          & $\Delta$ & {\color{red}0.97} & {\color{red}1.40} & {\color{red}0.84} \\
    \bottomrule
    \end{tabular}%
  \label{tab:diffStru-2}%
\end{table}%


==> iccv/section_tab/tab_diffStru.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table*}[htbp]
  \centering
  \caption{The Top-1 Accuracy (\%) of different knowledge distillation methods on the validation set of CIFAR-100~\cite{krizhevsky2009learning}. The teacher and student have distinct architectures. The KD methods are sorted by the types, i.e., feature-based and logit-based. We apply our logit standardization to the existing logit-based methods and use $\Delta$ to show its performance gain. The values in {\color{blue}blue} denote slight enhancement and those in {\color{red}red} non-trivial enhancement.}
    \begin{tabular}{llcccccccccc}
    \toprule
    \multirow{4}[2]{*}{Type} & \multirow{2}[1]{*}{Teacher} & ResNet32$\times$4 & ResNet32$\times$4 & ResNet32$\times$4 & ResNet32$\times$4 & ResNet32$\times$4 & WRN-40-2 & WRN-40-2 & WRN-40-2 & VGG13 & ResNet50 \\
          &       & 79.42 & 79.42 & 79.42 & 79.42 & 79.42 & 75.61 & 75.61 & 75.61 & 74.64 & 79.34 \\
          & \multirow{2}[1]{*}{Student} & SHN-V1 & SHN-V2 & WRN-40-2 & WRN-16-2 & VGG8  & SHN-V1 & ResNet8$\times$4 & MN-V2 & MN-V2 & MN-V2 \\
          &       & 70.50 & 71.82 & 75.61 & 73.26 & 70.36 & 70.50 & 72.50 & 64.60 & 64.60 & 64.60 \\
    \midrule
    \multirow{6}[2]{*}{Feature} & FitNet~\cite{romero2014fitnets} & 73.59 & 73.54 & 77.69 & 74.70 & 72.91 & 73.73 & 74.61 & 68.64 & 64.16 & 63.16 \\
          & RKD~\cite{park2019relational}   & 72.28 & 73.21 & 77.82 & 74.86 & 72.84 & 74.21 & 75.26 & 69.27 & 64.52 & 64.43 \\
          & CRD~\cite{tian2019contrastive}   & 75.11 & 75.65 & 78.15 & 75.65 & 73.54 & 76.05 & 75.24 & 70.28 & 69.73 & 69.11 \\
          & OFD~\cite{heo2019comprehensive}   & 75.98 & 76.82 & 79.25 & 76.17 & 73.85 & 75.85 & 74.36 & 69.92 & 69.48 & 69.04 \\
          & ReviewKD~\cite{chen2021distilling} & 77.45 & 77.78 & 78.96 & 76.11 & 74.35 & 77.14 & 74.34 & 71.28 & 70.37 & 69.89 \\
          & SimKD~\cite{chen2022knowledge} & 77.18 & 78.39 & 79.29 & 77.17 & 75.76 & 75.65 & 75.29 & 70.10 & 69.44 & 69.97 \\
    \midrule
    \multirow{9}[3]{*}{Logit} & KD~\cite{hinton2015distilling}    & 74.07 & 74.45 & 77.70 & 74.90 & 72.73 & 74.83 & 73.97 & 68.36 & 67.37 & 67.35 \\
          & KD+Ours & 74.44 & 75.56 & 77.92 & 75.26 & 73.23 & 75.64 & 77.11 & 69.23 & 68.61 & 69.02 \\
          & $\Delta$ & 0.37  & 1.11  & 0.22  & 0.36  & 0.50  & 0.81  & 3.14  & 0.87  & 1.24  & 1.67 \\
\cmidrule{2-12}          & KD+CTKD~\cite{li2022curriculum}  & 74.71 & 75.37 & 77.66 & 74.57 & 72.47 & 75.64 & 74.61 & 68.34 & 68.50 & 68.67 \\
          & KD+CTKD+Ours & 74.85 & 76.18 & 77.99 & 75.16 & 73.51 & 76.32 & 77.03 & 69.53 & 68.98 & 69.36 \\
          & $\Delta$ & 0.14  & 0.81  & 0.33  & 0.59  & 1.04  & 0.68  & 2.42  & 1.19  & 0.48  & 0.69 \\
\cmidrule{2-12}          & DKD~\cite{zhao2022decoupled}   & 76.45 & 77.07 & 78.46 & 75.70 & 74.48 & 76.70 & 75.56 & 69.28 & 69.71 & 70.35 \\
          & DKD+Ours & 76.77 & 77.37 & 78.95 & 76.19 & 74.61 & 76.95 & 76.75 & 70.01 & 69.98 & 70.45 \\
          & $\Delta$ & 0.32  & 0.30  & 0.49  & 0.49  & 0.13  & 0.25  & 1.19  & 0.73  & 0.27  & 0.10 \\
    \bottomrule
    \end{tabular}%
  \label{tab:diffStru}%
\end{table*}%


==> iccv/section_tab/tab_imagenet-mn2.tex <==
% Table generated by Excel2LaTeX from sheet 'imagenet'
\begin{table*}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{cccccccccccccc}
    \toprule
    \multicolumn{3}{c}{KD Type} & \multicolumn{5}{c}{Feature}           & \multicolumn{6}{c}{Logit} \\
    \midrule
          & Teacher & Sudent & AT    & OFD   & CRD   & ReviewKD & SimKD & KD    & KD+Ours & CTKD  & CTKD+Ours & DKD   & DKD+Ours \\
    \midrule
    top-1 & 76.16 & 68.87 & 69.56 & 71.25 & 71.37 & 72.56 & 72.25 & 70.50 & 72.18 & 71.16 & 72.20 & 72.05 & 72.85 \\
    top-5 & 92.86 & 88.76 & 89.33 & 90.34 & 90.41 & 91.00 & 90.86 & 89.80 & 90.80 & 90.11 & 91.00 & 91.05 & 91.18 \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%


==> iccv/section_tab/tab_imagenet-rn18.tex <==
% Table generated by Excel2LaTeX from sheet 'imagenet'
\begin{table*}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{ccc|ccccc|cccccc}
    \toprule
    \multicolumn{3}{c}{KD Type} & \multicolumn{5}{c}{Feature}           & \multicolumn{6}{c}{Logit} \\
    \midrule
          & Teacher & Student & AT    & OFD   & CRD   & ReviewKD & SimKD & KD    & KD+Ours & CTKD  & \multicolumn{1}{c}{CTKD+Ours} & DKD   & DKD+Ours \\
    \midrule
    top-1 & 73.31 & 69.75 & 70.69 & 70.81 & 71.17 & 71.61 & 71.59 & 71.03 & 71.42 & 71.38 &       & 71.70 & 71.88 \\
    top-5 & 91.42 & 89.07 & 90.01 & 89.98 & 90.13 & 90.51 & 90.48 & 90.05 & 90.29 & 90.27 &       & 90.41 & 90.45 \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%


==> iccv/section_tab/tab_vit.tex <==

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[tp]
% \vspace{1mm}
\footnotesize
\tabcolsep=0.4mm
\renewcommand\arraystretch{0.9} 
  \centering
  \caption{The Top-1 Accuracy (\%) of KD methods on CIFAR-100. Teacher is ResNet56. Hie. indicates if model is hierarchy structure. No logs and codes for Auto-KD are available yet. 
  }
  \vspace{-2mm}
    \begin{tabular}{l|cc|cccc|cc}
    \toprule
         Student & Hie. & Size & Train & AT    & LG~\cite{li2022Locality}   & {\scriptsize Auto-KD~\cite{li2023Automated}} & KD    & KD+Ours \\
    \midrule
    DeiT-Ti & \ding{55} & 5M & 65.08 & 73.51 & 78.15 & \textbf{78.58} & 73.25 & \underline{78.55}\(_{\textcolor{c6}{\tiny+5.30}}\) \\
    T2T-ViT-7 & \ding{55} & 4M & 69.37 & 74.01 & 78.35 & \textbf{78.62} & {74.15} & \underline{78.43}\(_{\textcolor{c6}{\tiny+4.28}}\) \\
    PiT-Ti & \ding{52} & 5M & 73.58 & 76.03 & 78.48 & \underline{78.51} & {75.47} & \textbf{78.76}\(_{\textcolor{c6}{\tiny+3.29}}\) \\
    PVT-Ti & \ding{52} & 13M & 69.22 & 74.66 & 77.07 & \underline{77.48} & {73.60} & \textbf{78.43}\(_{\textcolor{c6}{\tiny+4.83}}\) \\
    \bottomrule
    \end{tabular}%
  \label{tab:vit}%
  % \vspace{-1.mm}
\end{table}%

